PS-Sim: A Framework for Scalable Simulation of Participatory Sensing Data

Emergence of smartphone and the participatory sensing (PS) paradigm have paved the way for a new variant of pervasive computing. In PS, human user performs sensing tasks and generates notifications, typically in lieu of incentives. These notifications are real-time, large-volume, and multi-modal, which are eventually fused by the PS platform to generate a summary. One major limitation with PS is the sparsity of notifications owing to lack of active participation, thus inhibiting large scale real-life experiments for the research community. On the flip side, research community always needs ground truth to validate the efficacy of the proposed models and algorithms. Most of the PS applications involve human mobility and report generation following sensing of any event of interest in the adjacent environment. This work is an attempt to study and empirically model human participation behavior and event occurrence distributions through development of a location-sensitive data simulation framework, called PS-Sim. From extensive experiments it has been observed that the synthetic data generated by PS-Sim replicates real participation and event occurrence behaviors in PS applications, which may be considered for validation purpose in absence of the groundtruth. As a proof-of-concept, we have used real-life dataset from a vehicular traffic management application to train the models in PS-Sim and cross-validated the simulated data with other parts of the same dataset.

==> sections/1_introduction.tex <==
%% Insert your citation key below as it is in main.bib file to generate References in IEEE format.
 Items with same author is shown in "---"\\
 \\

\noindent An article \cite{anarticle}\\
A book \cite{abook}\\
A series \cite{bookseries}\\
Someone's thesis \cite{thesis}\\
Some technical report \cite{report}\\
A collection \cite{collection}\\
Visited website \cite{website}\\
Accepted for publication \cite{acceptedpub}\\
Submitted for publication \cite{unpub}\\
Not published \cite{notpub}\\
Conversation \cite{conv}





==> sections/references.tex <==
\begin{thebibliography}{13}
\scriptsize

\bibitem{burke06} J. A. Burke, D. Estrin, M. Hansen, A. Parker, N. Ramanathan, S. Reddy, and M. B. Srivastava. ``Participatory Sensing''. \emph{Center for Embedded Network Sensing}, 2006.
\bibitem{wang13} X. Wang, W. Cheng, P. Mohapatra, and T. Abdelzaher. ``ARTSense: Anonymous Reputation and  Trust in Participatory Sensing'', \emph{IEEE International Conference on Computer Communications (INFOCOM)}, pp. 2517-2525, 2013.
\bibitem{wang15} D. Wang, T. Abdelzaher, and L. Kaplan. ``Social Sensing: Building Reliable Systems on Unreliable Data''. \emph{Morgan Kaufmann}, 2015.
\bibitem{barnwal16} R. P. Barnwal, N. Ghosh, S. K. Ghosh, and S. K. Das. ``Enhancing Reliability of Vehicular Participatory Sensing Network: A Bayesian Approach''. \emph{IEEE International Conference on Smart Computing (SMARTCOMP)}, pp. 1-8, 2016.
\bibitem{gao15} L. Gao, F. Hou, and J. Huang. ``Providing Long-term Participation Incentive in Participatory Sensing''. \emph{IEEE International Conference on Computer Communications (INFOCOM)}, pp. 2803-2811, 2015.
\bibitem{restuccia16} F. Restuccia, S. K. Das, and J. Payton. ``Incentive Mechanisms for Participatory Sensing: Survey and Research Challenges''. \emph{ACM Transactions on Sensor Networks (TOSN)}, vol. 12, no. 2, 2016.
\bibitem{cardone14} G. Cardone, A. Cirri, A. Corradi, and L. Foschini. ``The Participact Mobile Crowd Sensing Living Lab: The Testbed for Smart Cities''. \emph{IEEE Communications Magazine}, vol. 52, no. 10, pp. 78-85, 2014.
\bibitem{gedeon15} J. Gedeon and I. Schweizer. ``Understanding Spatial and Temporal Coverage in Participatory Sensor Networks'', \emph{IEEE International Conference on Local Computer Networks (LCN) Workshops}, pp. 699-707, 2015
\bibitem{zhang12} W. Zhang, B. Zhu, L. Zhang, J. Yuan, and I. You. ``Exploring Urban Dynamics based on Pervasive Sensing: Correlation Analysis of Traffic Density and Air Quality''. \emph{IEEE International Conference on Innovative Mobile and Internet Services in Ubiquitous Computing (IMIS)}, pp. 9-16, 2012.
\bibitem{foell13} S. Foell, G. Kortuem, R. Rawassizadeh, S. Phithakkitnukoon, M. Veloso, and C. Bento. ``Mining Temporal Patterns of Transport Behavior for Predicting Future Transport Usage''. \emph{ACM Conference on Ubiquitous Computing (UbiComp)}, pp. 1239-1248, 2013.
\bibitem{reddy08} S. Reddy, K. Shilton, J. Burke, D. Estrin, M. Hansen, and M. Srivastava. ``Evaluating Participation and Performance in Participatory Sensing''. \emph{International Workshop on Urban, Community, and Social Applications of Networked Sensing Systems (UrbanSense08)}, vol. 4, 2008.
\bibitem{tomasini17} M. Tomasini, B. Mahmood, F. Zambonelli, A. Brayner, and R. Menezes. ``On the Effect of Human Mobility to the Design of Metropolitan Mobile Opportunistic Networks of Sensors''. \emph{Elsevier Pervasive and Mobile Computing}, 2017.
\bibitem{zhao14} K. Zhao, M. Musolesi, P. Hui, W. Rao, and S. Tarkoma. ``Explaining the Power-Law Distribution of Human Mobility through Transportation Modality Decomposition'' \emph{Nature Scientific Reports}, 2015.
\end{thebibliography} 
